Exploiting high-contrast Stokes preconditioners to efficiently solve incompressible fluid-structure interaction problems

In this work, we develop a new algorithm to solve large-scale incompressible time-dependent fluid--structure interaction (FSI) problems using a matrix-free finite element method in arbitrary Lagrangian--Eulerian (ALE) frame of reference. We derive a semi-implicit time integration scheme which improves the geometry-convective explicit (GCE) scheme for problems involving the interaction between incompressible hyperelastic solids and incompressible fluids. The proposed algorithm relies on the reformulation of the time-discrete problem as a generalized Stokes problem with strongly variable coefficients, for which optimal preconditioners have recently been developed. The resulting algorithm is scalable, optimal, and robust: we test our implementation on model problems that mimic classical Turek benchmarks in two and three dimensions, and investigate timing and scalability results.

==> algorithms/gce-pc.tex <==
\DontPrintSemicolon
\KwData{$\ur^{n-i},\vr^{n-i},\wr^{n-i}, \quad i = 1,\dots,k$}
\KwResult{$\ur^{n},\vr^{n},\wr^{n}$}

\Begin{
$\wre :=\wr^{n-1}$ \;
 \vspace*{0.5\baselineskip}
\SetKw{kwIn}{in}
\For{$j$ \kwIn {$( \predictor, \corrector \; )$ } } {
$\ure  :=  \gamma\timestep \wre-\sum\limits _{i=1}^{k}\alpha_{i}\ur^{n-k}$ \Comment*{Explicit step}
$\mapae =\Id+ \ure,\qquad \Oe=\mapae(\Or)$ \Comment*{New geometry}
 \vspace*{1\baselineskip}
Find  $\vci \in H^{1}(\Oe)$ and $\implicit{\pressure}\in L^2(\Oe):$ \Comment*{Implicit step}
\begin{equation}
\label{eq:ggce:implicit}
\begin{cases}
\begin{array}{lll}
{a}_{j}(\vci,\testv)+{b}(\testv,\implicit{\pressure}) & =g_{j}(\testv)& \forall\testv\in H_{D}^{1}(\Oe),\\
{b}(\vci,q) & = g_p(q)\,& \forall q\in L^{2}(\Oe).
\end{array}
\end{cases}
\end{equation}\;
 \vspace*{0.25\baselineskip}
$\wri :=\Ext(\vri)$ \Comment*{Extension}
$\wre :=\wri$
 }
 
 \vspace*{0.25\baselineskip}
 
 $\vr^n:=\vri ,\qquad  \wr^{n} :=\wri$\;
 
 $\ur^n:=\gamma\timestep \wr^{n}-\sum\limits _{i=1}^{k}\alpha_{i}\ur^{n-i}$ \Comment*{Displacement recovery}
 }
